Analytic MMSE Bounds in Linear Dynamic Systems with Gaussian Mixture Noise Statistics

Using state-space representation, mobile object positioning problems can be described as dynamic systems, with the state representing the unknown location and the observations being the information gathered from the location sensors. For linear dynamic systems with Gaussian noise, the Kalman filter provides the Minimum Mean-Square Error (MMSE) state estimation by tracking the posterior. Hence, by approximating non-Gaussian noise distributions with Gaussian Mixtures (GM), a bank of Kalman filters or Gaussian Sum Filter (GSF), can provide the MMSE state estimation. However, the MMSE itself is not analytically tractable. Moreover, the general analytic bounds proposed in the literature are not tractable for GM noise statistics. Hence, in this work, we evaluate the MMSE of linear dynamic systems with GM noise statistics and propose its analytic lower and upper bounds. We provide two analytic upper bounds which are the Mean-Square Errors (MSE) of implementable filters, and we show that based on the shape of the GM noise distributions, the tighter upper bound can be selected. We also show that for highly multimodal GM noise distributions, the bounds and the MMSE converge. Simulation results support the validity of the proposed bounds and their behavior in limits.

==> ChaptAppend.tex <==
\label{sec:ProofCovariance}
The state error covariance matrix for filter \(ij\) at iteration \(k\) can be evaluated as follows:
\begin{align}
P_{k|k}^{ij}= & \textrm{cov}\left(\mathbf{x}_k - \mathbf{\hat{x}}_{k|k}^{ij}\right) \\
= & \textrm{cov}\left(\mathbf{x}_k - \left(\mathbf{\hat{x}}_{k|k-1}^{ij} +W_k^{ij} \boldsymbol{\nu}_{k}^{ij} \right) \right) \\
= & \textrm{cov}\left(\mathbf{x}_k - \left(\mathbf{\hat{x}}_{k|k-1}^{ij} +W_k^{ij} \left(\mathbf{z}_k -H_k\mathbf{\hat{x}}_{k|k-1}^{ij} - \mathbf{b}_k^{j}\right) \right) \right) \\
= & \textrm{cov}\left(\mathbf{x}_k - \left(\mathbf{\hat{x}}_{k|k-1}^{ij} +W_k^{ij} \left(H_k\mathbf{x}_k + \mathbf{w}_k -H_k\mathbf{\hat{x}}_{k|k-1}^{ij} - \mathbf{b}_k^{j}\right) \right) \right) \\
= & \textrm{cov}\left(\left(I -W_k^{ij}H_k \right) \left(\mathbf{x}_k -\mathbf{\hat{x}}_{k|k-1}^{ij}\right) - W_k^{ij}\mathbf{w}_k + W_k^{ij}\mathbf{b}_k^{j}  \right) \\
= & \left(I -W_k^{ij}H_k \right) P_{k|k-1}^{ij} \left(I -W_k^{ij}H_k \right)^T + W_k^{ij} R_k^{ij} {W_k^{ij}}^T \\
= & P_{k|k-1}^{ij} - W_k^{ij}H_kP_{k|k-1}^{ij} 
- P_{k|k-1}^{ij}H_k^T{W_k^{ij}}^T+ W_k^{ij}H_kP_{k|k-1}^{ij}H_k^T{W_k^{ij}}^T+ W_k^{ij} R_k^{ij} {W_k^{ij}}^T \\
= & P_{k|k-1}^{ij} - W_k^{ij}H_kP_{k|k-1}^{ij} 
- P_{k|k-1}^{ij}H_k^T{W_k^{ij}}^T+ W_k^{ij}\left(H_kP_{k|k-1}^{ij}H_k^T+ R_k^{ij}\right) {W_k^{ij}}^T\\
= & P_{k|k-1}^{ij} - W_k^{ij}H_kP_{k|k-1}^{ij} 
- P_{k|k-1}^{ij}H_k^T{W_k^{ij}}^T+ W_k^{ij}S_k^{ij}{W_k^{ij}}^T
\end{align}

==> ChaptMMSEProof.tex <==
The MMSE state estimation is by definition equal to~\cite{bar2001estimation,poor_introduction_1994}:
\begin{align}
\hat{\mathbf{{x}}}_{k}^{\mathrm{MMSE}}  = \arg \min_{\hat{\mathbf{{x}}}_{k}}E \left\lbrace \left(\mathbf{{x}}_{k}- \hat{\mathbf{{x}}}_{k} \right)^T\left(\mathbf{{x}}_{k}- \hat{\mathbf{{x}}}_{k} \right) |\mathbf{{z}}_{1:k} \right\rbrace.
\end{align}
Setting the gradient of the mean-squared-error to zero, we will have:
\begin{align}
\label{eq:MMSEGradient}
 \nabla_{\hat{\mathbf{{x}}}_{k}}E \left\lbrace \left(\mathbf{{x}}_{k}- \hat{\mathbf{{x}}}_{k} \right)^T\left(\mathbf{{x}}_{k}- \hat{\mathbf{{x}}}_{k} \right) |\mathbf{{z}}_{1:k} \right\rbrace = 2 \left(E \left\lbrace \mathbf{{x}}_{k} |\mathbf{{z}}_{1:k} \right\rbrace-{\hat{\mathbf{{x}}}_{k}}\right) = 0.
\end{align}
Hence, using Eq.~\eqref{eq:GSFmergedposterior} and Eq.~\eqref{eq:MMSEGradient} we can write
\begin{align}
\label{eq:MMSEestimateProof}
\hat{\mathbf{{x}}}_{k}^{\mathrm{MMSE}} =E \left\lbrace \mathbf{{x}}_{k} |\mathbf{{z}}_{1:k} \right\rbrace.
\end{align}

==> ChaptSurvey.tex <==
Bayesian tracking techniques can be used for estimating unobservable state of a dynamic system from observable measurements, by approximating the posterior distribution or belief function. For linear dynamic systems with Gaussian noises, the posterior density is Gaussian and its sufficient statistics can be optimally tracked using Kalman filter~\cite{ho_bayesian_1964,arulampalam_tutorial_2002}. However, for the case of non-Gaussian noises, approximations should be made to provide suboptimal solutions~\cite{arulampalam_tutorial_2002}. Gaussian Mixtures can be used for approximating the non-Gaussian  distributions, as they can provide asymptotically unbiased estimations~\cite{1962KernelDensityEstimation}, with the desired precision~\cite[Chapter8; Lemma 4.1]{anderson1979optimal}. Additionally, they enable the analytic evaluation of posterior distributions and provide closed-form representations for the belief function. Hence, they have been used to model the prior ~\cite{anderson1979optimal,alspach_nonlinear_1972,sorenson_recursive_1971,flament_particle_2004,maybeck_multiple_2005,morelande_manoeuvring_2005,lehn-schioler_parzen_2004,bilik_optimal_2005}, likelihood~\cite{huber_hybrid_2007,huber_efficient_2007}, predictive density~\cite{huber_hybrid_2007_Other,stordal_bridging_2011,yang_gaussian_2010,ali-loytty_efficient_2008}, noise distributions~\cite{bar2001estimation,GSPFkotecha_gaussian_2003,chen_mixture_2000,alspach_nonlinear_1972,sorenson_recursive_1971,schoenberg_posterior_2012,kemouche_gmm_2010,bilik_mmse-based_2010,sun_mixture_2004,ali-loytty_box_2010,ali-loytty_convergence_2008,faubel_split_2009,shao_improving_2008,xiang_modified_2008,wang_novel_2012,bilik_optimal_2005,daeipour_interacting_1995}, or directly the posterior distribution~\cite{ito_gaussian_2000,GPFkotecha_gaussian_2003,crisan_generalised_2013,schoenberg_posterior_2012,terejanu_adaptive_2011,foo_combining_2011,bilik_maneuvering_2010,ali-loytty_efficient_2008,faubel_split_2009,xiang_modified_2008,wang_novel_2012,djuric_density_2004,schrempf_efficient_2007,wu_quasi-gaussian_2006,bethel_pdf_2010}. 

With GM representations of noise distributions in dynamic systems, the state can be tracked and estimated by parallel Kalman filters, or Gaussian Sum Filters (GSF). In~\cite{anderson1979optimal}, it is shown that starting with a finite GM prior, and additive white Gaussian noise, the predictive and posterior distributions will also be GM. When the process and measurement noises are Gaussian, the number of mixands in the posterior remains the same. However, for non-Gaussian noises approximated by GMs, the number of mixands in the posterior grows exponentially over time. Hence, suitable Gaussian Mixture reduction algorithms should be used. One of the most used methods for reduction, is simply removing the clusters with smaller weights, and only keeping the mixands with significant weights. This is the approach used in~\cite{alspach_nonlinear_1972,sorenson_recursive_1971} and it is attractive due to its low complexity. Another reduction scheme based on removing smaller mixands, can be similar to the resampling algorithm in particle filters. This is the approach used in~\cite{GSPFkotecha_gaussian_2003,crisan_generalised_2013,andrieu_particle_2002}. Alternatively, in~\cite{ali-loytty_convergence_2008,ali-loytty_box_2010,ali-loytty_efficient_2008} a \textit{forgetting and merging} algorithm is proposed, where the mixands with weights smaller than a threshold are removed, and the clusters  with close enough moments are merged. Alternatively, the GM distribution can be viewed as a single Gaussian conditioned on a latent variable determining the mode or the cluster. Hence, by tracking the latent variable, only the corresponding cluster of the GM is kept~\cite{chen_mixture_2000,sun_mixture_2004} and the other mixands are simply removed.

In~\cite{bar2001estimation,GPFkotecha_gaussian_2003,shao_improving_2008,morelande_manoeuvring_2005,djuric_density_2004,wu_quasi-gaussian_2006,bolic_study_2010} instead of removing any clusters, they are all merged to a single Gaussian distribution at the end of each iteration. For higher order models, where the mode conditioning also includes the history of the state\footnote{e.g. in Generalized Pseudo Bayesian estimator of second order (GPB2) the mode conditioning is on the current and previous state}, Interacting Multiple Models (IMM) can be used to merge the clusters by starting from different initial conditions for each filter in the bank. IMM is less computationally complex when compared with GPB2, because unlike GPB2 which requires \(r^2\) filters for \(r\) initial conditions, IMM requires only \(r\) filters at each iteration. Hence, it has been widely used for second order models~\cite{bar2001estimation,foo_combining_2011,morelande_manoeuvring_2005,daeipour_interacting_1995}. Instead of merging the clusters regardless of the shape of the approximated distribution, in~\cite{faubel_split_2009} the clusters are merged in the unlikely regions of the distribution, and they are split in the likely regions, so that the mixture reflects the distribution more accurately using less number of mixands. 

Another class of reduction algorithms provide solutions by minimizing a cost function, which can be based on Kullback-Leibler divergence~\cite{schoenberg_posterior_2012,bilik_mmse-based_2010}, a least squares error function~\cite{kemouche_gmm_2010}, or an integral squares error~\cite{maybeck_multiple_2005}. Other forms of cost functions can also be used for this purpose. However, these schemes usually suffer from high complexity as they use numerical methods for minimizing a function.

Alternatively, Expectation Maximization (EM) algorithm can be used to simultaneously predict and reduce the Gaussian Mixture~\cite{huber_efficient_2007,bilik_maneuvering_2010,xiang_modified_2008,wang_novel_2012,bilik_optimal_2005}, e.g. by running the EM algorithm on synthetically generated data~\cite{bilik_optimal_2005,bilik_maneuvering_2010}.

Table~\ref{tab:references} provides a summary of these papers.

\begin{table}[!t]
\centering
\caption{Related work}
\label{tab:references}
\begin{tabular}{l|l|l|l}
	&	functions	&	GMM distribution	&	Mixture Reduction Scheme	\\ \hline
\cite{bar2001estimation}	&	Linear	&	Process noise	&	GPB1; GPB2; IMM	\\ \hline
\cite{anderson1979optimal}	&	Non-linear	&	Prior distribution	&	Constant number of mixands	\\ \hline
\cite{ito_gaussian_2000}	&	Non-linear 	&	Prior distribution	&	Constant number of mixands	\\ \hline
\cite{GPFkotecha_gaussian_2003}	&	Non-linear	&	Posterior	&	Merge to 1	\\ \hline
\cite{GSPFkotecha_gaussian_2003}	&	Non-linear	&	Process noise	&	Resampling 	\\ \hline
\cite{chen_mixture_2000}	&	Linear	&	Process and measurement noise	&	Latent variable is tracked	\\ \hline
\cite{crisan_generalised_2013}	&	Non-linear	&	Posterior	&	Resampling-correction step	\\ \hline
\cite{alspach_nonlinear_1972}	&	Non-linear	&	Process noise, Prior distribution	&	removing smaller clusters; merging the clusters with close means	\\ \hline
\cite{sorenson_recursive_1971}	&	Linear	&	Process and measurement noise, Prior distribution	&	removing smaller clusters	\\ \hline
\cite{andrieu_particle_2002}	&	Linear	&	everything is Gaussian	&	resampling	\\ \hline
\cite{schoenberg_posterior_2012}	&	Non-linear	&	Measurement noise	&	Minimizing cost function (based on KL divergence)	\\ \hline
\cite{huber_hybrid_2007}	&	Non-linear	&	Likelihood distribution	&	Constant number of mixands	\\ \hline
\cite{huber_efficient_2007}	&	Non-linear	&	Likelihood distribution	&	simultaneous prediction and reduction 	\\ \hline
\cite{huber_hybrid_2007_Other}	&	Non-linear	&	Predictive distribution	&	Constant number of mixands	\\ \hline
\cite{flament_particle_2004}	&	Non-linear	&	Prior distribution	&	Constant number of mixands	\\ \hline
\cite{kemouche_gmm_2010}	&	Non-linear	&	Process and measurement noise	&	Minimizing cost function (least squares error function)	\\ \hline
\cite{terejanu_adaptive_2011}	&	Non-linear	&	Posterior	&	Constant number of mixands	\\ \hline
\cite{stordal_bridging_2011}	&	Linear/Non-linear	&	Predictive distribution	&	Constant number of mixands	\\ \hline
\cite{bilik_mmse-based_2010}	&	Linear	&	Process and measurement noise	&	greedy EM algorithm to minimize the KL divergence	\\ \hline
\cite{maybeck_multiple_2005}	&	Linear	&	Prior distribution	&	Minimizing cost function (Integral Square Error (ISE))	\\ \hline
\cite{foo_combining_2011}	&	Linear/Non-linear	&	Posterior	&	IMM	\\ \hline
\cite{yang_gaussian_2010}	&	Non-linear	&	Posterior	&	Constant number of mixands	\\ \hline
\cite{sun_mixture_2004}	&	Linear	&	Process and measurement noise	&	Constant number of mixands	\\ \hline
\cite{bilik_maneuvering_2010}	&	Non-linear	&	Posterior	&	EM	\\ \hline
\cite{ali-loytty_box_2010}	&	Linear/Non-linear	&	Process and measurement noise	&	forgetting and/or merging	\\ \hline
\cite{ali-loytty_convergence_2008}	&	Linear/Non-linear	&	Process and measurement noise	&	forgetting and/or merging	\\ \hline
\cite{ali-loytty_efficient_2008}	&	Non-linear	&	Predictive distribution, Posterior	&	forgetting and/or merging; resampling	\\ \hline
\cite{faubel_split_2009}	&	Non-linear	&	Process and measurement noise, Posterior	&	splitting in likely parts, merging in unlikely parts	\\ \hline
\cite{shao_improving_2008}	&	Non-linear	&	Process noise	&	Merge to 1	\\ \hline
\cite{morelande_manoeuvring_2005}	&	Non-linear	&	Prior distribution	&	Merge to 1; IMM	\\ \hline
\cite{freitas_diagnosis_2004}	&	Linear	&	Posterior	&	Constant number of mixands	\\ \hline
\cite{xiang_modified_2008}	&	Non-linear	&	Process and measurement noise, Posterior	&	EM	\\ \hline
\cite{wang_novel_2012}	&	Non-linear	&	Process and measurement noise, Posterior	&	EM	\\ \hline
\cite{djuric_density_2004}	&	Linear	&	Posterior	&	Merge to 1	\\ \hline
\cite{schrempf_efficient_2007}	&	Non-linear	&	Posterior	&	Constant number of mixands	\\ \hline
\cite{lehn-schioler_parzen_2004}	&	Non-linear	&	Prior distribution	&	Constant number of mixands	\\ \hline
\cite{bilik_optimal_2005}	&	Linear	&	Process noise, Prior distribution	&	EM	\\ \hline
\cite{daeipour_interacting_1995}	&	Linear/Non-linear	&	Measurement noise	&	IMM	\\ \hline
\cite{wu_quasi-gaussian_2006}	&	Non-linear	&	Posterior	&	merge to one
\end{tabular}
\end{table}
